Pressure dependence of intra- and interlayer excitons in 2H-MoS$_2$ bilayers

The optical and electronic properties of multilayer transition metal dichalcogenides differ significantly from their monolayer counterparts due to interlayer interactions. The separation of individual layers can be tuned in a controlled way by applying pressure. Here, we use a diamond anvil cell to compress bilayers of 2H-MoS$_2$ in the gigapascal range. By measuring optical transmission spectra, we find that increasing pressure leads to a decrease in the energy splitting between the A and interlayer exciton. Comparing our experimental findings with ab initio calculations, we conclude that the observed changes are not due to the commonly assumed hydrostatic compression. This effect is attributed to the MoS$_2$ bilayer adhering to the diamond, which reduces in-plane compression. Moreover, we demonstrate that the distinct real-space distributions and resulting contributions from the valence band account for the different pressure dependencies of the inter- and intralayer excitons in compressed MoS$_2$ bilayers.

==> backup.tex <==

\subsection{Conclusion}

We measured pressure-dependent optical transmission spectra of bilayer 2H-\ce{MoS2} crystals using a diamond anvil cell. To explain our experimental results, we calculated structural changes of the \ce{MoS2} crystal under different types of compression and investigated their influence on the samples optical absorption. By doing so we showed how to interpret experimental results from 2D materials inside a diamond anvil cell despite the non-trivial interaction of sample and substrate under pressure. We observe that intra- and interlayer excitons are influenced differently by crystal compression, which we attribute to an increase of interlayer interactions under pressure. Our work facilitates the successful application of high pressure experiments within the field of 2D materials.

%Intro
Molybdenum disulphide (\ce{MoS2}) is a layered van-der-Waals material and a member of the transition metal dichalcogenides (TMDCs) \cite{frisenda_naturally_2020}. Their electronic band structure (i.e. being metallic, semimetallic, semiconducting) varies depending on their chemical formula and crystal structure \cite{kuc_electronic_2015}. \ce{MoS2} in the 2H-phase is a two dimensional (2D) semiconductor \cite{mueller_exciton_2018, frindt_physical_1963}. Since it was discovered that \ce{MoS2} (and others) are direct semiconductors in their monolayer form \cite{mak_atomically_2010}, single layers have drawn the majority of scientific interest in the last years \cite{chiu_synthesis_2015}. Due to their large binding energies \cite{he_tightly_2014}, excitons dominate the opto-electronic properties in these materials. The excitons are strongly influenced by the surrounding of the monolayer. This effect has been demonstrated by depositing the monolayer on top of different substrates. The enhanced screening due to the substrates leads to spectral shifts  of the excitons \cite{chernikov_exciton_2014, cadiz_excitonic_2017, ajayi_approaching_2017}. Similarly, in crystals consisting of two (or more) TMDC layers, the interaction between adjacent layers has a large effect on the optoelectronic properties \cite{novoselov_2D_2016}. In particular, interlayer excitons can form, which consist of an electron and a hole residing in different layers. Interlayer excitons have also been found in heterostructures of TMDCs \cite{rivera_interlayer_2018}. Interestingly, they are very prominent in 2H-\ce{MoS2} homo-bilayers \cite{gerber_interlayer_2019}. Here, the interlayer exciton has a comparatively large oscillator strength and is energetically separated from intralayer excitons, rendering this material a promising test bed.


\noindent{\bf Monolage experimentell, mal gucken, was daraus wird}
First, we focus on the \ce{MoS2} monolayer and the changes of the optical properties caused by the compression of an individual layer. The emission and absorption spectra at different pressures are shown in Fig. X, respectively. The A and B excitons in the transmission spectra show a blueshift with increasing pressure at a rate of +10 meV/GPa. The separation of the two excitonic lines stays almost constant for all pressure values. For higher pressures, the resonances get broader and weaker. They are ultimately not discernible at highest pressures (above 8 GPa). The photoluminescence (PL) emission spectrum at ambient pressure (Fig. X) shows the well-known single-line emission of the direct (\(KK\)) A exciton. With increasing pressure, the emission blueshifts, in unison to the transmission results. With increasing pressure, a second broad line arises at lower energies, which is clearly visible at pressures above 5 GPa around 1.71 eV and redshifts down to 1.65 eV at 9 GPa. With increasing pressure its intensity increases, while the PL intensity of the A exciton reduces strongly. We attribute this second emission line to the indirect \(K\Lambda\) exciton . It arises as the conduction band (CB) minimum at the \(\Lambda\) point crosses the \(K\) point minimum. They shift in opposite directions under pressure, as seen in the calculated band structures (figure X). An earlier work has reported this crossover at lower pressures (around 1.9 GPa) and with no direct evidence for the coexistence of the two excitonic species \cite{fu_k-_2017}. We attribute the deviation in the shift rates and the transition pressure to the use of different substrates in that study as opposed to our (Si instead of diamond). We interpret the transfer of PL intensity from the initial resonance to the new one as a consequence of photo excited electrons scattering to the energetically lowest state, which is \(\Lambda\) instead of \(K\) at elevated pressures. The combined emission intensity reduces since an increasing portion of indirect excitons are created, which need to interact with a phonon in order to recombine and emit a photon.


The emission spectrum of the bilayer at ambient pressure shows the direct (\(KK\)) as well as the indirect (\(\Gamma K\)) exciton transition. The \(KK\) transition stays almost constant in energy with increasing pressure as found also in the transmission spectra. The indirect transition however strongly redshifts, which is due to the strong shift of the valence (VB) maximum at the \(\Gamma\) point, which is very sensitive to interlayer interactions. In contrast to the \ce{MoS2} monolayer, the PL intensity of the \ce{MoS2} bilayer does not decrease further with increasing pressure although the band gap shrinks and it becomes an even more indirect semiconductor. [This indicates that the formation of \(KK\) excitons is not limited by holes scattering to the \(\Gamma\) point, but rather by electrons scattering to the \(\Lambda\) point.] Above 5 GPa, the PL intensity even increases, which indicates that more direct excitons get created than at ambient pressure. It seems with increasing pressure the formation of \(KK\) exciton becomes more favourable. Since this is not the case in the monolayer this could possibly be attributed to the increased binding energy of the interlayer exciton in the bilayer. 


We show that the band crossing in the conduction band of monolayer \ce{MoS2} under pressure is accompanied by a gradual transition of direct to indirect exciton formation. In the bilayer we find an increased PL intensity under pressure which might indicate a low energy excitonic state at the K point which is not present in the monolayer.

In Fig.~\ref{fig:spectra}, the theoretically calculated absorption spectra for pure out-of-plane compression (\ref{fig:spectra}b) and hydrostatic pressure (\ref{fig:spectra}c) are shown. Applying hydrostatic pressure to the bilayer leads to a shift to higher energies, opposed to a shift to lower energies observed in the case of out-of-plane compression. This contrasting behaviour is mainly caused by the differences in the in-plane structure. While the interlayer distance $d$ as well as the \ce{S}-\ce{S} distance behave quite similar in both cases, decreasing approximately exponentially, the lattice constant $a$ shrinks linearly from \SI{3.18}{\AA} under zero pressure to \SI{3.11}{\AA} under \SI{10}{GPa} hydrostatic pressure. Our geometrical results are in accordance with former publications \cite{fan_electronic_2015, peelaers_elastic_2014, yengejeh_effect_2020}. The influence of the in-plane structure on the optical spectra is also observed at \ce{MoS2} monolayers, where a biaxial stretching leads to a shift to smaller energies, which is in accordance with our results\cite{frisenda_biaxial_2017, heissenbuettel_nature_2019}. The behaviour of the band structure under hydrostatic pressure helps to understand the energy shifts within the corresponding absorption spectra (Fig. \ref{fig:bandstructure}a). The direct gap at K becomes larger with increasing pressure. It grows approximately linear from \SI{2.53}{eV} to \SI{2.75}{eV} under \SI{10}{GPa} and is the reason for the shift to higher energies of the three excitons. 
In contrast to the hydrostatic pressure, the gap at K decreases under out-of-plane pressure to \SI{2.43}{eV} at \SI{10}{GPa} (Fig. \ref{fig:bandstructure}b). This happens not linearly, but in the same way as the decrease of the interlayer distance. The result is the shift to lower energies of the excitation energies. Furthermore, the valence band (VB) splitting growths as in the former case and the conduction band (CB) splitting does not change its value significantly. So, the relation between the shifts are the same as before, while their absolute values are different. 
